Multiaccurate Proxies for Downstream Fairness

We study the problem of training a model that must obey demographic fairness conditions when the sensitive features are not available at training time -- in other words, how can we train a model to be fair by race when we don't have data about race? We adopt a fairness pipeline perspective, in which an "upstream" learner that does have access to the sensitive features will learn a proxy model for these features from the other attributes. The goal of the proxy is to allow a general "downstream" learner -- with minimal assumptions on their prediction task -- to be able to use the proxy to train a model that is fair with respect to the true sensitive features. We show that obeying multiaccuracy constraints with respect to the downstream model class suffices for this purpose, provide sample- and oracle efficient-algorithms and generalization bounds for learning such proxies, and conduct an experimental evaluation. In general, multiaccuracy is much easier to satisfy than classification accuracy, and can be satisfied even when the sensitive features are hard to predict.

==> New Folder With Items/experiments.tex <==
In this section, we perform an empirical evaluation of our proxy training algorithms. Observe that our theorems are predicated on two assumptions that are either difficult to verify or else do not hold exactly in practice:
\begin{enumerate}
    \item Our class $\Gs$ contains a good proxy. We cannot verify this without demonstrating one, which we have to do by training a good proxy. 
    \item We have a cost sensitive classification oracle for $\Hs$ (and in the non-linear case, also for $\Gs$). In practice we do not have ``oracles'' and most learning problems are NP-complete, but we have good heuristics that we can use in place of our oracles.
\end{enumerate}

Our experiments are aimed at verifying the utility of our algorithms, even in the simple case in which we take $\Gs$ to be the set of linear regression functions and $\Hs$ to be the set of linear threshold functions.

\subsection{Methodology}

\label{sec:methodology_preiminaries}

\subsubsection{Weighted Binary Sample Transformation}
\label{sec:swt}

To use a real-valued proxy with standard downstream algorithms for fair machine learning algorithms, many of which assume sensitive features are binary or categorical, we transform a dataset with real-valued sensitive features (see \S\ref{sec:data}) into a dataset with twice as many samples, each of which is paired with a \textit{binary} group membership and sample weight (see Definition~\ref{def:swt} and Claim~\ref{clm:swt}). We note that many learning algorithms are already equipped to handle sample weights, so our transformed dataset fits nicely into existing methods. 

\subsubsection{Paired Regression Classifier}
\label{sec:prc}

For the oracle $CSC(\Hs)$, we experiment with the paired regression classifier (PRC) used in \cite{minimax2} and \cite{gerrymandering}. The PRC produces a \emph{linear threshold function}, just as logistic regression does -- see Definition~\ref{def:PRC}.

\subsubsection{Reductions algorithm for error parity}
\label{sec:reductions_accuracy_parity}

The reductions algorithm for error parity was introduced in \cite{agarwal2018reductions} as a method of producing randomized ensembles of classifiers that achieve high population accuracy while satisfying accuracy parity between sensitive groups. The algorithm takes a relaxation parameter $\gamma \in [0, 1]$ that specifies the maximum allowable difference in error between any two sensitive groups. We implemented the algorithm and augmented it to support arbitrary sample weights. See Definition~\ref{def:reductions_error_parity} for a precise specification. 

\subsection{Experimental Process}
\label{sec:exp_process}

We performed a variety of experiments on real, fairness-sensitive datasets, taking $\Gs$ to be the model class of linear regression functions and $\Hs$ to be the class of linear threshold functions. We compared the performance of a proxy trained with our algorithm (``$\Hs$-proxy'') to the performance achieved using the true sensitive features (``true labels''), a binary proxy in the form of a logistic regression model (``baseline proxy''), and a real-valued proxy in the form of a linear regression model (``mean-squared error (MSE) proxy''). We evaluated the performance of the models produced by the downstream learner for each type of proxy on both group error disparity (with respect to the true sensitive features) and overall population accuracy.

For the three types of proxies and the true labels we performed the following:
\begin{enumerate}
    \item Train the proxy.
    \item If the proxy is real-valued ($\Hs$- or MSE proxy), apply the Weighted Binary Sample Transformation to the dataset.
    \item Train a downstream learner using the reductions algorithm for accuracy parity (described in Section~\ref{sec:reductions_accuracy_parity}) to produce a relaxation curve of models over 10 values of $\gamma \in \{0, 0.005, 0.001, \dots, 0.045\}$.
\end{enumerate}

We plot the performance of the proxies with respect to population error and error disparity between the sensitive groups. The error disparity is plotted with respect to the \textit{true sensitive features}, even for the downstream models that only have access to the proxy features during training.

\subsection{Implementation}
\label{sec:implementation}

We implemented a generic and slightly simplified version of our proxy training algorithm in PyTorch that (approximately) solves our constrained optimization problem via gradient descent. Our implementation leverages auto-differentiation to avoid solving for gradients explicitly in closed form and allows us to select $\Gs$ as an arbitrary architecture multi-layer perceptron (MLP). In particular, this permits $\Gs$ as the class of linear models--which is equivalent to the class of one-layer perceptrons--but also enables the use of our algorithm to train more complex proxies. We also support an arbitrary downstream learner class $\Hs$,  given an algorithm for training regression models in $\Hs$. \footnote{See the Section~\ref{sec:appendix_implementation} of the appendix for a full report of the implementation details and hyperparameter selection.}

\subsection{Data}
\label{sec:data}

We primarily relied on the recently published American Community Survey (ACS) datasets and tasks from~\cite{DBLP:journals/corr/abs-2108-04884}. Rather than looking at the entire United States, we focused our analysis on data from New York state, which we found was sufficiently large to admit excellent out-of-sample generalization. For each task, we examined three sensitive features: sex, age, and race. Because we focus on binary sensitive attributes, we transformed age and race into binary features; we thresholded age at 40 years, and we treated race as a white/non-white binary indicator. All downstream models were trained to make predictions without having access to \textit{any} of the three sensitive features, regardless of which feature the model enforced fairness with respect to. Categorical features were converted into one-hot encoded vectors and the dimensionality $d$ was computed before one-hot encoding. The table below summarizes the tasks used in our experiments. Full details about each prediction task are specified in the appendix in Section~\ref{sec:appendix_datasets}.
 
\begin{table}[ht]
\centering
\begin{tabular}{|l|c|c|l|l|l|}
\hline
Dataset   & \multicolumn{1}{l|}{Sample Count} & \multicolumn{1}{l|}{$d$} & Label                                                                       & Sensitive Feature(s)     \\  
\hline

ACSEmployment & 196104 & 12 & Employment & Race, sex, age \\
\hline
ACSIncome & 101270 & 4 & Income > \$50K & Race, sex, age \\
\hline
ACSIncomePovertyRatio & 196104 & 15 & Income-Poverty Ratio < 250\% & Race, sex, age \\
\hline
ACSMobility & 39828 & 17 & Same address one year ago & Race, sex, age \\
\hline
ACSPublicCoverage & 71379 & 15 & Health Insurance & Race, sex, age \\
\hline
ACSTravelTime & 89145 & 8 & Commute > 20 minutes& Race, sex, age \\
\hline
\end{tabular}
\label{tab:data}
\end{table}

\subsection{Results Overview}

\begin{itemize}

  \item A linear proxy trained with our algorithm often serves as an excellent substitute for the true sensitive features and enables us to train downstream models that attain high population accuracy while enforcing fairness constraints with respect to the true sensitive features. This performance is robust to relaxations in fairness constraints of the downstream learner.
  
  \item Models trained on $\Hs$-proxies almost never performed worse than those trained on a naive baseline--which for linear models is a logistic regression trained to predict the binary sensitive feature of each instance--and often performed far better. 
   
  \item Nearly all downstream models we experimented with generalized extremely well out-of-sample with respect to both fairness and accuracy. In fact, for most experiments the in-sample and out-of-sample plots appear nearly identical in terms of both the shape of the tradeoff curves and the values they span. This generalization performance can likely be attributed to the choice to use linear-complexity $\Gs$ and $\Hs$ rather than more complex classes. Further experimentation is necessary before assuming good out-of-sample generalization for non-linear proxies or downstream learners. 
  
  \item On some tasks, the $\Hs$-proxy failed to serve as a good substitute for the true sensitive features, resulting in a downstream model that violated the intended fairness constraints. However, in each of our experiments where this occurred, the failure of the proxy could be detected at training time. We address these failures in more detail in the appendix (Section~\ref{sec:addressing_failures}). 
    
   \item Often, the MSE proxy--which is a simple linear regression model without the additional multi-accuracy constraints--serves as a performant proxy. This empirical finding justifies the use of the MSE in the objective function of our constrained optimization problem as a heuristic for finding good solutions. We also find that the real-valued MSE proxy often out-performs the naive binary-valued baseline. This is predicted by our Claim \ref{clm:existence}, which proves that this will work whenever the conditional distribution on the protected feature can be well approximated by a linear function. 

\end{itemize}


\subsection{Plots}
\label{sec:plots}

In this section we will analyze the experimental results on the ACSIncome dataset on the three sensitive features race, age, and sex. The ACSIncome dataset is an improved version of the popular Adult dataset, making these experiments more easily contextualized with those in the existing literature compared to the other ACS tasks. Moreover, we found these three tasks had diverse results that demonstrated the capability of our proxy algorithm while also revealing some of its shortcomings in practice. The remaining experiments and plots, including those on which the proxy failed more dramatically, can be found in the appendix in Section~\ref{sec:appendix_plots}. \footnote{Since our downstream models are randomized ensembles, we report all statistics \textit{in expectation} over these ensembles. This means that we can create linear combinations of models to trace a Pareto frontier, which is plotted as a dotted line.}

\subsubsection{ACS-Income-Race}
Fig.~\ref{fig:acs_income_race} displays nearly ideal results supporting the theory. In sample, downstream models trained on true sensitive features exhibit the best tradeoff curve, followed by the $\Hs$-proxy, and then the MSE proxy, all three of which exhibit a sensible tradeoff between error disparity and population error. The $\Hs$-proxy induces a tradeoff curve with similar shape to that of the true labels, but with ${\sim}$0.003 greater error disparity and ${\sim}$0.01 greater error. The curve of the MSE proxy is similar in shape to that of the $\Hs$-proxy but with accuracy ${\sim}0.002$ less than the $\Hs$-proxy. The least disparate model induced by the MSE proxy is equally accurate to that of the $\Hs$-proxy, but marginally less disparate. The baseline proxy exhibits the worst downstream performance, with a clustered tradeoff curve that is Pareto dominated by models from all other proxies. For \textit{any} model trained with the baseline proxy, we can improve accuracy by more than 0.01 without increasing disparity by switching to some model trained with our $\Hs$-proxy. 

Out-of-sample behavior of all models is quite similar to in-sample, though the maximum disparity for all curves decreases from  ${\sim}0.025$ to ${\sim}0.02$ and the least disparate models trained on the true labels increase disparity from  ${\sim}0$ to ${\sim}0.0025$. 
 
\begin{figure*}[h]
    \centering
    \includegraphics[width=0.7\textwidth]{plots_final/acs-income-race.png}
    \captionsetup[subfigure]{labelformat=empty, belowskip=0pt}
    \caption{Proxy results on the ACSIncome dataset with race as sensitive feature}
    \label{fig:acs_income_race}
\end{figure*}

\subsubsection{ACS-Income-Age}
In Fig.~\ref{fig:acs_income_age} we observe that the downstream performance of models trained on the $\Hs$-proxy are nearly identical to that of the models trained with the true sensitive features, indicating success for our proxy algorithm. Models trained on both of these proxies exhibit a clean tradeoff between error and fairness; the least disparate models achieve error disparity near 0 and population error slightly under 0.29, and the most disparate models accept error disparity ${\sim}$0.05 to achieve population error near 0.25. The baseline and MSE proxies induce similar tradeoffs but are unable to induce downstream models with error disparity lower than  ${\sim}$0.01. This indicates success of the $\Hs$-proxy's multi-accuracy constraints in enforcing downstream accuracy parity -- its least disparate model achieves error disparity near 0. Out of sample, the performance of each model is nearly identical to its performance in sample. 

\begin{figure*}[h]
    \centering
    \includegraphics[width=0.7\textwidth]{plots_final/acs-income-age.png}
        \captionsetup[subfigure]{labelformat=empty, belowskip=0pt}
    \caption{Proxy results on the ACSIncome dataset with age as sensitive feature}
    \label{fig:acs_income_age}
\end{figure*}

\subsubsection{ACS-Income-Sex}
In Fig.~\ref{fig:acs_income_sex} we observe that the downstream performance of the models trained on the $\Hs$-proxy is quite close to that of the the true labels, although the minimum disparity it achieves is greater by about 0.007. This indicates that the $\Hs$-proxy is not a perfect substitute for the true labels, although it is still quite good. As we relax fairness constraints, this disparity in accuracy gap between the models trained on the $\Hs$-proxy and those trained on the true labels shrinks, and the left endpoints of both curves are nearly identical in terms of error and disparity. Of the three proxies, the baseline proxy achieves the lowest error disparity of ${\sim}$0.0025 on the training data, but it comes at the cost of significantly lower accuracy. At the same levels of disparity, the model trained on the $\Hs$-proxy is more accurate than the model trained on the baseline by ${\sim}$0.01, and for error disparity values greater than ${\sim}$0.0075, the $\Hs$-proxy Pareto dominates the baseline in terms of both accuracy and  accuracy gap. Generalization is quite good for all models: the shape of each curve and the range of values spanned is consistent in and out of sample, although nearly all models are slightly more disparate out-of-sample. \footnote{The one exception to this is the rightmost point on the curve of models corresponding to the baseline proxy, which achieves slightly lower error disparity out-of-sample. However, given that the other models trained on the baseline proxy have worse out-of-sample performance than in-sample, we suspect this empirical improvement is simply noise that, by luck, worked in the proxy's favor.}



\begin{figure*}[h]
    \centering
    \includegraphics[width=0.7\textwidth]{plots_final/acs-income-sex.png}
        \captionsetup[subfigure]{labelformat=empty, belowskip=0pt}
    \caption{Proxy results on the ACSIncome dataset with sex as sensitive feature}
    \label{fig:acs_income_sex}
\end{figure*}


==> New Folder With Items/facct_linear.tex <==
Our follow-the-perturbed-leader based algorithm can handle an arbitrary proxy class $\Gs$, so long as we have an oracle for optimizing over it. But the algorithm can simplify substantially when the primal optimization problem is convex in its parameters, as it is when we choose $\Gs$ to be the set of linear proxies.  In this section we consider the case in which $\hat{z}(x;\theta)$ is a linear regression of $x$ on the true sensitive features $z$, taking the form $\hat{z}(x;\theta) = \theta x$. Because both $\hat{z}$ and its negation are convex in $\theta$, we can find such a proxy by implementing a two-player game in which the Proxy Learner uses Online Projected Gradient Descent, and the Auditor best responds by appealing to an oracle over $\Hs$, as in Algorithm~\ref{alg:ftpl}. We summarize Online Projected Gradient Descent below.

\paragraph{Online Projected Gradient Descent}
Online Projected Gradient Descent is a no-regret online learning algorithm which we can formulate as a two-player game over $T$ rounds. At each round $t \leq T$, a Learner selects an action $\theta^t$ from its action space $\Theta \subset \Re^d$ (equipped with the $L_2$ norm) and an Auditor responds with a loss function $\ell^t: \Theta \to \R_{\ge 0}$. The learner's loss at round $t$ is $\ell^t(\theta^t)$. If the learner is using an algorithm $A$ to select its action each round, then the learner wants to pick $A$ so that the regret $R_A(T) := \sum_{t=1}^{T} \ell^t (\theta^t) - \min_{\theta \in \Theta} \sum_{i=1}^{T} \ell^t(\theta)$ grows sublinearly in $T$. When $\Theta$ and the loss function played by the Auditor are convex, the Learner may deploy Online Projected Gradient Descent (Algorithm~\ref{alg:descent}) to which the Auditor best responds. In this scenario, each round $t$, the Learner selects $\theta^{t+1}$ by taking a step in the opposite direction of the gradient of that round's loss function, and $\theta^{t+1}$ is projected into the feasible action space $\Theta$. Pseudocode and the regret bound are included below.

\begin{algorithm}[t]
\KwIn{learning rate $\eta$}
Initialize the learner $\theta^1 \in \Theta$\;
\For{$t=1, 2, \ldots$}{
Learner plays action $\theta^{t}$\;
Adversary plays loss function $\ell^t$\;
Learner incurs loss of $\ell^t (\theta^t)$\;
Learner updates its action:
$\theta^{t+1} = \text{Proj}_{\Theta} \left( \theta^{t} - \eta \nabla \ell^{t} (\theta^{t}) \right)$
}
\caption{Online Projected Gradient Descent}
\label{alg:descent}
\end{algorithm}

\begin{thm}[Regret for Online Projected Gradient Descent \cite{zinkevich}]\label{thm:gdregret} 
    Suppose $\Theta \subseteq \R^d$ is convex, compact and has bounded  diameter $D$: $\sup_{\theta, \theta' \in \Theta} \left\Vert \theta - \theta' \right\Vert_2 \le D$. Suppose for all $t$, the loss functions $\ell^t$ are convex and that there exists some $G$ such that $\left\Vert \nabla \ell^t (\cdot) \right\Vert_2 \le G$. Let $\mathcal{A}$ be Algorithm~\ref{alg:descent} run with learning rate $\eta = D/(G \sqrt{T})$. We have that for every sequence of loss functions $(\ell^1, \ell^2, \ldots, \ell^T)$ played by the adversary, $R_\mathcal{A}(T) \le GD \sqrt{T}$.
\end{thm}

\paragraph{Specifying and Solving the Linear Program}
Many aspects of our setup for Algorithm~\ref{alg:ftpl} are shared here. In particular, we once again focus on solving the minimax problem \eqref{eq:minimaxp} by viewing it as a two player zero sum game. The primal player (the Learner) controls $p_k$, but this time explicitly through the parameter $\theta$, and the dual player (the Auditor) controls $\lambda$. We continue to utilize no-regret dynamics; now, however, the Proxy Learner plays Online Projected Gradient Descent, and the Auditor with strategies in $\Lambda = \{ \lambda = (\lambda_0, \lambda') \in \R^d: | \lambda_0 | \le C_0, \Vert \lambda' = (\lambda_{h,j})_{h,j} \Vert_1 \le C \}$ best responds by appealing to a cost sensitive classification oracle over the class $H$ (CSC($H$)). Upper bounds ($C_0$ and $C$) on the dual variable components are again set to guarantee convergence.

Our algorithm is described in Algorithm~\ref{alg:EqualErrors} and its guarantee is given in Theorem~\ref{thm:linear}. The algorithm once again returns a distribution over $\Gs$, but because $\hat{z}$ is now convex in $\theta$, we can simply return an average over $\theta$ as our final model. This is the approach we take in our experiments. In contrast to the previous algorithm, the Auditor calls upon $CSC(\Hs)$ to maximize the exact costs without additional noise. Note that in practice, we need to use a heuristic to estimate $CSC(\Hs)$, as such an oracle is generally not available in practice; more information is given in Section~\ref{sec:experiments}.

\begin{algorithm}
\SetAlgoLined
\KwIn{ Data set $\{x_i,y_{ij},z_i\}_{i=1}^{n} \forall j \in [m]$, target proxy parameter $\alpha$, upper bound $M$ on proxy values, upper bound $B$ on magnitude of proxy gradient values, groups $k \in [K]$, dimension of parameter vector $d$, diameter of $\Theta$ space $D$;
}
Set dual variable upper bound: $C = \lceil \left( M^2(1+nM) + 2\alpha \sum_{i=1}^n z_{ik}(1+nM))^{-1} \right)/ \left( \alpha \sum_{i=1}^n z_{ik} \right) \rceil$\;
Set iteration count: $T = \lceil \left( d D (1+nM)\left( 2MB + nCB \left( \sum_{i=1}^{n} z_{ik}\right)^{-1}\right) / \left( \alpha \sum_{i=1}^n z_{ik} \right) \right)^2 \rceil$\;
\For{$k=1$ \textbf{to} $K$}{
\For{$t=1$ \textbf{to} $T$}{
    Set $\eta = t^{-1/2}$\;
    $h^*, j^* = \argmax_{h \in \Hs, j \in [m]} |\sum_{i=1}^n \left(z_{ik} - \hat{z}_{k} (x_i; \theta_k) \right) \1 \left[ h(x_i) \neq y_{ij} \right]| $\;
    \If{$|\sum_{i=1}^n \left(z_{ik} - \hat{z}_{k} (x_i; \theta_k)\right) \1 \left[ h^*(x_i) \neq y_{ij^*} \right]| \geq |\frac{\sum_{i=1}^n \hat{z}_{k} (x_i; \theta_k)}{\sum_{i=1}^n z_{ik}} - 1|$}{
    $\lambda_{h^*,j^*} = C \cdot \sign \left( \sum_{i=1}^n \left(z_{ik} - \hat{z}_{k} (x_i; \theta_k)\right) \1 \left[ h^*(x_i) \neq y_{ij^*} \right]\right) $\;
    }
    \Else{$\lambda_0 = C \cdot \sign \left( \frac{\sum_{i=1}^n \hat{z}_{k} (x_i; \theta_k)}{\sum_{i=1}^n z_{ik}} - 1\right)$}
    Set all other $\lambda$ to 0\;

    $\frac{\delta L}{\delta \theta_k}=\frac{2}{n}\sum_{i=1}^{n} \nabla_{\theta_k} \hat{z}_k(x_i;\theta_k)\cdot \left( \hat{z}_k(x_i;\theta_k)- z_{ik} \right) + \lambda_0 \frac{\sum_{i=1}^n \nabla_{\theta_k}\hat{z}_{k} (x_i; \theta_k)}{\sum_{i=1}^n z_{ik}} - \lambda_{h^*,j^*} \sum_{i=1}^n \nabla_{\theta_k} \hat{z}_{k} (x_i; \theta_k) \1 \left[ h^*(x_i) \neq y_{ij^*} \right]$\;
$\theta_k^{(t+1)} = \theta_k^{(t)}-\eta^{t} \frac{\delta L}{\delta \theta_k}$\;
}
}
\KwOut{$\hat{p}$ = uniform distribution over $\{ \hat{z}(\cdot; \theta^1)$,...,$\hat{z}(\cdot; \theta^T) \}$}
\caption{Learning a Linear Proxy}
\label{alg:EqualErrors}
\end{algorithm} 

\begin{thm}[Learning a Linear $\alpha$-Proxy]
\label{thm:linear}
Fix any $\alpha$. Suppose $\Hs$ has finite VC dimension, and $\Gs$ has finite pseudo-dimension. Suppose $\Delta (\Gs)^K$ contains a $0$-proxy. Then given access to oracle $CSC(\Hs)$, Algorithm~\ref{alg:EqualErrors} returns a distribution $\hat{p} \in \Delta (\Gs)^K$ such that $\hat{z} (x) \triangleq \E_{g \sim \hat{p}} \left[ g(x) \right] = (1/T) \sum_{t=1}^T \hat{z}_t (x)$ is an $\alpha$-proxy.
\end{thm}



==> New Folder With Items/facct_nonlinear.tex <==
\section{Learning a Proxy from Data}
\label{sec:general}

We now give a general oracle  efficient algorithm that the Proxy Learner can use to learn a proxy, whenever the underlying proxy class $\Gs^K$ is expressive enough to contain one. Our algorithm is in fact a general method for obtaining a \textit{multiaccurate} regression function $\hat z$ with respect to an arbitrary collection of sets --- we instantiate it with sets defined by the error regions of classifiers $h \in \Hs$. In contrast to the algorithms for multiaccurate learning given by \cite{multiaccuracy,multiaccuracy2}, our algorithm has the advantage that it need not be able to evaluate which sets a new example is a member of at test time (but has the disadvantage that it must operate over a sufficiently expressive model class). This is crucial, because we will not know whether a new example $x$ falls into the error region of a classifier $h$ before learning its label.  

Our derivation proceeds as follows. First, we rewrite the constraints in Program~\eqref{eqn:program1} as a large linear program. We then appeal to strong duality to derive the Lagrangian of the linear program. We note that computing an approximately optimal solution to the linear program corresponds to finding approximate equilibrium strategies for both players in the game in which one player ``The Learner'' controls the primal variables and aims to minimize the Lagrangian value, and the other player ``The Auditor'' controls the dual variables and aims to maximize the Lagrangian value.

Finally, if we construct our algorithm in such a way that it simulates repeated play of the Lagrangian game such that both players have sufficiently small regret, we can apply  Theorem~\ref{thm:noregret} to conclude that our empirical play converges to an approximate equilibrium of the game. In our algorithm, the Learner approximately best responds to the mixed strategy of the Auditor -- who plays \textit{Follow the Perturbed Leader (FTPL)} \citep{kalai}, described in the appendix. Note that it is the functions played by the Learner that will eventually form the proxy output by the  \textit{Proxy Learner}. Furthermore, our algorithm will be \textit{oracle efficient}: it will make polynomially many calls to oracles that solve ERM problems over $\Hs$ and $\Gs$. The specific types of oracles that we need are defined as follows.

\begin{definition}[Cost Sensitive Classification Oracle for $\Hs$]
An instance of a Cost Sensitive Classification problem, or a $CSC$ problem, for the class $\Hs$ is given by a set of $n$ tuples $\{x_i,c_i^0,c_i^1 \}_{i=1}^{n}$ such that $c_i^l$ corresponds to the cost for predicting label $l$ on sample $x_i$. Given such an instance as input, a $CSC (\Hs)$ oracle finds a hypothesis $h \in \Hs$ that minimizes the total cost across all points:
$
h \in \argmin_{h' \in \Hs} \sum_{i=1}^{n}\left[h'(x_i)c_i^1 + (1-h'(x_i))c_i^0\right]
$.
\end{definition}

\begin{definition}[Empirical Risk Minimization Oracle for $\Gs$]
\label{def:erm}
An empirical risk minimization oracle for a class $\Gs$ (abbreviated $ERM (\Gs)$) takes as input a data set $S$ consisting of $n$ samples and a loss function $L$, and finds a function $g \in \Gs$ that minimizes the empirical loss, i.e., $g \in \text{argmin}_{g' \in \Gs} \sum_{i=1}^{n} L(g',S_i)$.
\end{definition}

\ifdraft
\paragraph{Follow the Perturbed Leader} Follow the Perturbed Leader (FTPL) is a no-regret learning algorithm that can sometimes be applied -- with access to an oracle -- to an appropriately convexified learning space that is too large to run gradient descent over. It is formulated as a two-player game over $T$ rounds. At each round $t \leq T$, a learner selects an action $a^t$ from its action space $A \subset \{0,1\}^d$, and an auditor responds with a loss vector $\ell^t \in \Re ^d$. The learner's loss is the inner product of $\ell^t$ and $a^t$. If the learner is using an algorithm $A$ to select its action each round, then the learner wants to pick $A$ so that the regret $R_A(T) := \sum_{t=1}^{T} \langle \ell^t, a^t\rangle - \min_{a \in A} \sum_{i=1}^{T} \langle \ell^t, a^t \rangle$ grows sublinearly in $T$. Algorithm~\ref{alg:ftpl_pseudo} accomplishes this goal by perturbing the cumulative loss vector with appropriately scaled noise, and then an action is chosen to minimize the perturbed loss. Pseudocode and guarantees are stated below. 

\begin{algorithm}[h]
\KwIn{learning rate $\eta$}
Initialize the learner $a^1 \in A$\;
\For{t = 1,2, \ldots}{
Learner plays action $a^{t}$\;
Adversary plays loss vector $\ell^t$\;
Learner incurs loss of $\langle \ell^t, a^t \rangle$. Learner updates its action: $a^{t+1} = \argmin_{a \in A} \left\{ \left\langle \sum_{s \le t} \ell^s , a \right\rangle + \frac{1}{\eta} \left\langle \xi^t , a \right\rangle \right\}$ \;
where $\xi^t \sim Uniform \left( [0,1]^d \right)$, independent of every other randomness.
}
\caption{Follow the Perturbed Leader (FTPL)}
\label{alg:ftpl_pseudo}
\end{algorithm}

%The guarantees of Follow the Perturbed Leader are stated below.

\begin{thm}[Regret of FTPL \cite{kalai}]
\label{thm:ftpl}
    Suppose for all $t$, $\ell^t \in [-M,M]^d$. Let $\mathcal{A}$ be Algorithm~\ref{alg:ftpl_pseudo} run with learning rate $\eta = 1/(M \sqrt{dT})$. For every sequence of loss vectors $(\ell^1, \ell^2, \ldots, \ell^T)$ played by the adversary,  $\E \left[ R_\mathcal{A}(T) \right] \le 2 M d^{3/2} \sqrt{T}$, where expectation is taken with respect to the randomness in $\mathcal{A}$. 
\end{thm}
\else
\fi

\paragraph{Specifying the Linear Program.} To transform Program~\eqref{eqn:program1} into a linear program amenable to our two-player zero sum game formulation, we do the following: 1) We break the constraints of Program~\eqref{eqn:program1}, which are given as equality of fractions, into joint equality of their numerators and denominators. 2) We expand $\Gs$ to the set of distributions over $\Gs$: we will find a distribution $p \in \Delta (\Gs)$, where $\Delta (\Gs)$ is the set of probability distributions over $\Gs$, and further \textit{linearize} our objective function and constraints by taking expectations with respect to the variable $p \in \Delta (\Gs)$. 3) Finally, we ensure that we have \textit{finitely many} variables and constraints by assuming that $\Hs$ and $\Gs$ have bounded complexity. In particular, given a data set $S$, we can write constraints corresponding to every $h \in \Hs (S) \triangleq \{ (h(x_1), \ldots, h(x_n)): h \in \Hs\}$ where $\Hs(S)$ includes the set of all possible labelings induced by $\Hs$ on $S$. Note that as long as $\Hs$ has finite VC dimension $d_\Hs$, Sauer's Lemma implies $\vert \Hs (S) \vert = O(n^{d_\Hs})$, and therefore we will have only finitely many constraints. Second, instead of working with the entire class $\Gs$, for some appropriately chosen $\epsilon$, and given our data set $S$, we can optimize over (distributions over) an $\epsilon$-covering of $\Gs$ with respect to the data set $S$, which we call $\Gs (S)$. As long as the class $\Gs$ has finite pseudo-dimension $d_\Gs$, it is known that $|\Gs (S)| = O(\epsilon^{-d_\Gs})$, and therefore we reduce our primal variables from distributions over $\Gs$ to distributions over $\Gs (S)$ which will guarantee that we have finitely many variables in our optimization problem. We provide more details in the appendix. Given these considerations, we  formulate the constrained ERM problem of the PL as follows: for every group $k \in [K]$, the PL solves

\begin{mini}|l|
{p_k \in \Delta (\Gs (S))}{\frac{1}{n}\sum_{i=1}^{n} \E_{\hat{z}_k \sim p_k} \left[ \left( z_{ik} - \hat{z}_k (x_i) \right)^2 \right]}{}{}
\addConstraint{\frac{\sum_{i=1}^n \E_{\hat{z}_k \sim p_k} \left[ \hat{z}_{k} (x_i) \right]}{\sum_{i=1}^n z_{ik}} - 1 = 0 \;}{}{}
\addConstraint{
\sum_{i=1}^n \left( z_{ik} - \E_{\hat{z}_k \sim p_k} \left[ \hat{z}_{k} (x_i) \right]\right) \1 \left[ h(x_i) \neq y_{ij} \right] = 0, }{}{\; \forall j \in [m], \forall h \in \Hs (S)}
\label{eqn:programAlgos}
\end{mini}

We will solve this constrained optimization problem by simulating a zero sum two player game on the Lagrangian dual. Given dual variables $\lambda \in \R^d$ (where $d = 1 + m | H(S)|$) we have that the Lagrangian of Program~\eqref{eqn:programAlgos} is given by:
\begin{align}
L(\lambda,p_k) &= \frac{1}{n} \sum_{i=1}^{n} \E_{\hat{z}_k \sim p_k} \left[ \left( z_{ik} - \hat{z}_k (x_i) \right)^2 \right] + \E_{\hat{z}_k \sim p_k} \left[ \lambda_0\left(\frac{\sum_{i=1}^n \hat{z}_{k} (x_i)}{\sum_{i=1}^n z_{ik}} - 1\right) +\sum_{\substack{h \in \Hs (S) \\ j \in [m]}} \lambda_{h,j} \sum_{i=1}^n \left(z_{ik} - \hat{z}_{k} (x_i) \right) \1 \left[ h(x_i) \neq y_{ij} \right] \right]
\label{eqn:game}
\end{align}

Given the Lagrangian, solving linear program~\eqref{eqn:programAlgos} is equivalent to solving the following minimax problem:
\begin{equation}\label{eq:minimaxp}
\min_{p_k \in \Delta (\Gs (S))} \max_{\lambda \in \R^d} L(\lambda,p_k) = \max_{\lambda \in \R^d} \min_{p_k \in \Delta (\Gs (S))} L(\lambda,p_k)
\end{equation}
where the minimax theorem holds because the range of the primal variable, i.e. $\Delta (\Gs (S))$, is convex and compact, the range of the dual variable, i.e. $\R^d$, is convex, and that the Lagrangian function $L$ is linear in both primal and dual variables. Therefore we focus on solving the minimax problem \eqref{eq:minimaxp} which can be seen as a two player zero sum game between the primal player (the Learner) who is controlling $p_k$, and the dual player (the Auditor) who is controlling $\lambda$. Using  no-regret dynamics, we will have the Learner deploy its best response strategy in every round which will be reduced to a call to $ERM (\Gs)$ and let the Auditor with strategies in $\Lambda = \{ \lambda = (\lambda_0, \lambda') \in \R^d: | \lambda_0 | \le C_0, \Vert \lambda' = (\lambda_{h,j})_{h,j} \Vert_1 \le C \}$ play according to Follow the Perturbed Leader (FTPL). We place upper bounds ($C_0$ and $C$) on the components of the dual variable to guarantee convergence of our algorithm; note that the minimax theorem continues to hold in the presence of these upper bounds. We will set these upper bounds optimally in our algorithm to guarantee the desired convergence. 

Our algorithm is described in Algorithm~\ref{alg:ftpl} and its guarantee is given in Theorem~\ref{thm:ftplProxy}. The algorithm returns a distribution over $\Gs$, but we turn the distribution into a deterministic regression function that defines a proxy by taking the expectation with respect to that distribution. We note that the Auditor will employ FTPL for the constraints that depend on $h$, calling upon the cost sensitive classification oracle $CSC(\Hs)$. Given an action $\hat{z}_k$ of the Learner, we write $LC(\hat{z}_k)$ for the vector of costs for labelling each data point as 1. Note that this formulation allows us to cast our seemingly nonlinear problem as an $n$-dimension linear optimization problem, which we do by viewing our costs as the inner product of the outputs of a classifier $h$ on the $n$ points and the corresponding cost vector, derived in the appendix.


%Note that this formulation allows us to cast our seemingly nonlinear problem as an $n$-dimension linear optimization problem, which we do by viewing our costs as the inner product of the outputs of a classifier $h$ on the $n$ points and the corresponding cost vector.
%Given an action $\hat{z}_k$ of the Learner, we write $LC(\hat{z}_k)$ for the vector of costs for labelling each data point as 1. Note that this formulation allows us to cast our seemingly nonlinear problem as an $n$-dimension linear optimization problem, which we do by viewing our costs as the inner product of the outputs of a classifier $h$ on the $n$ points and the corresponding cost vector. See the Appendix for a derivation of the costs.

We denote the true distribution over $\lambda'$ maintained by the Auditor's FTPL algorithm by $Q_k^t$. Because $Q_k^t$ is a distribution over an exponentially large domain $(O(n^{d_\Hs}))$, we can only aim to represent a sparse version, which we do by efficiently sampling from $Q_k^t$; we call the empirical distribution $\hat{Q}_k^t$. We represent the Auditor's learned distribution over $\lambda_0$ by $P_k^t$, and we find that $P_k^t:=C_0\left(2Bern(p_k^t) - 1\right)$ is a scaled Bernoulli distribution with success probability $p_k^t$, where $p_k^t$ is given in Algorithm~\ref{alg:ftpl}. When we sample $\lambda= \left(\lambda_0,\lambda'\right)$ from the product distribution $P_k^t \times \hat{Q}_k^t$, this means that we are drawing $\lambda_0$ from $P_k^t$ and $\lambda'$ from $\hat{Q}_k^t$. The proof of Theorem~\ref{thm:ftplProxy}, below, is included in the appendix.


\begin{algorithm}
\SetAlgoLined
\KwIn{ Data set $\{x_i,y_{ij},z_i\}_{i=1}^{n} \forall j \in [m]$, target proxy parameter $\alpha$, target confidence parameter $\delta$, upper bound $M$ on proxy values, groups $k \in [K]$}
Set dual variable upper bounds: $C=C_0 = (M^2(1+nM)/2\alpha \sum_{i=1}^n z_{ik}) + 1$\;
Set iteration count: $T = \left\lceil \sqrt{2(1+nM)\left(n^{3/2}CM + C_0\frac{nM}{\sum_{i=1}^n z_{ik}}\right)/ \alpha\sum_{i=1}^n z_{ik}} \; \right\rceil$\;
Set sample count: $W = \left \lceil (1+nM)^2 n^2C^2M^2 \log(\frac{TK}{2\delta})/\left(\alpha \sum_{i=1}^n z_{ik} \right)^2 \; \right \rceil$\;
Set learning rates of FTPL: $\eta =\frac{1}{CM} \sqrt{\frac{1}{nT}}\;$, $\;\eta' = \frac{\sum_{i=1}^n z_{ik}}{C_0nM} \sqrt{\frac{1}{T}}$\;
\For{$k=1$ \textbf{to} $K$}{
Initialize $\hat{z}_k^0=\bar{0}$\;
\For{$t=1$ \textbf{to} $T$}{
\For{$w=1$ \textbf{to} $W$}{
Draw a random vector $\xi^w$ uniformly at random from $[0,1]^{n}$\;
Use oracle $CSC(\Hs)$ to compute:
$(h^{w,t}, j^{w,t}) = \argmin_{h \in H, j \in [m]} - \sum_{t' < t}|\langle LC_j(\hat{z}_k^{t'}),h \rangle| + \frac{1}{\eta} \langle\xi^w,h\rangle$\;
Let $\lambda'^{w,t}$ be defined as $\lambda^{w,t}_{h,j} = sign(2\1 \left[ \langle LC_{j^{w,t}}(\hat{z}_k^{t}),h^{w,t}\rangle > 0 \right] - 1) \times C \1 \left[h = h^{w,t},j = j^{w,t} \right]$\;
}

Let $\hat{Q}_k^t$ be the empirical distribution over $\lambda'^{w,t}$\;
Set distribution over $\lambda_0^t$ : $P_k^t = C_0\left(2Bern(p_k^t) - 1\right)$ where $p_k^t = \min(1,-\eta'(\frac{\sum_{i=1}^n \hat{z}_{k} (x_i)}{\sum_{i=1}^n z_{ik}} - 1)\1\left[\frac{\sum_{i=1}^n \hat{z}_{k} (x_i)}{\sum_{i=1}^n z_{ik}} -1 < 0 \right])$\;
The Learner best responds: $\hat{z}_k^t = \argmin_{\hat{z}_k \in \Gs} \mathbb{E}_{\lambda \sim P_k^t \times \hat{Q}_k^t} L(\hat{z}_k, \lambda)$ by calling $ERM(\Gs)$.
}
}
\KwOut{$\hat{p}$ = uniform distribution over $\{ \hat{z}^1$,...,$\hat{z}^T \}$}
\caption{Learning a Proxy}
\label{alg:ftpl}
\end{algorithm}

\begin{thm}[$\alpha$-Proxy for $m$ labeling functions taken from $\F$]
\label{thm:ftplProxy}
Fix any $\alpha$, and $\delta$. Suppose $\Hs$ has finite VC dimension, and $\Gs$ has finite pseudo-dimension. Suppose $\Delta (\Gs)^K$ contains a $0$-proxy. Then given access to oracles $CSC(\Hs)$ and $ERM(\Gs)$, we have that with probability at least $1-\delta$, Algorithm~\ref{alg:ftpl} returns a distribution $\hat{p} \in \Delta (\Gs)^K$ such that $\hat{z} (x) \triangleq \E_{g \sim \hat{p}} \left[ g(x) \right] = \frac{1}{T} \sum_{t=1}^T \hat{z}_t (x)$ is an $\alpha$-proxy. 

\end{thm}


==> New Folder With Items/facct_preliminaries.tex <==
Let $\Omega = \X \times \Z \times \Y$ be an arbitrary data domain. Each data point is a triplet $\omega = (x,z,y)$, where $x \in \X$ is the feature vector excluding the sensitive attributes, $z \in \Z$ is a vector of sensitive attributes, and $y \in \Y = \{0,1\}$ is the binary label. In this paper we take $\Z = \{0,1\}^K$, and every $z \in \Z$ is a $K$-dimensional binary vector representing which groups (out of $K$ groups) an individual is a member of. For instance, in a case with $K=4$ groups, an individual with $z = (0,1,0,1)$ is a member of the second and fourth groups. We will use $z_k$ to denote the $k$th entry of $z$.

We assume there exists a distribution $\Ps$ over the unlabeled data domain $\X \times \Z$. We assume the labels are generated by functions in some domain $\F \subseteq \{ f: \X \times \Z \to \Y \}$. In other words, for any data point $\omega = (x,z,y) \in \Omega$, there exists a function $f \in \F$ such that $y = f(x,z)$. This is without loss of generality if we make no assumptions on the complexity of $\F$ --- in this case, functions $f$ can be randomized and represent arbitrary conditional label distributions, and will be the setting we operate in when we assume there is a distribution over $\F$. Alternately, we can make assumptions about the capacity of $\F$, and then aim to form good proxies for \textit{every} labelling function in $\F$. The data generation process can be viewed as first drawing $(x,z)$ from $\Ps$, and then letting $y = f(x,z)$ for some $f \in \F$. We \textit{may} additionally assume there exists a probability distribution $\Qs$ over $\F$. More details are discussed later on.

Our primary goal in this paper is to learn a proxy for $z$ as a function of features $x$,  which we write as  $\hat{z}$, such that any downstream classifier satisfies a variety of fairness constraints with respect to the learned proxy $\hat{z}$ if and only if it satisfies the same fairness constraints with respect to the true underlying $z$, up to small approximation.  Let $\Gs \subseteq \{ g: \X \to [0,M] \}$ be a class of functions that map a feature vector $x \in \X$ to a real-valued number in $[0,M]$. Given $\Gs$, our goal will be to learn $\hat{z} = (\hat{z}_1, \ldots, \hat{z}_K)$ such that for all $k$, $\hat{z}_k \in \Gs$. The $k$th component of $\hat{z}$ can be interpreted as a real-valued predictor for $z_k$.

We assume the downstream learning task for which we want to guarantee fairness can be cast as learning over a hypothesis class $\Hs \subseteq \{ h: \X \to \Y \}$. Thus the goal of the DLs will be to learn $h \in \Hs$ such that $h$ satisfies some statistical notion of fairness. These fairness notions generally require that a statistic of the learned classifier be (approximately) equalized across different groups. While our methods will apply to a broad class of fairness notions including statistical parity and equalized false positive and negative rates (see the appendix for details), in the body we focus on  \textit{equalized error} fairness  which requires that the error rate of the learned classifier be (approximately) equalized across groups. In other words, $h \in \Hs$ satisfies equalized error fairness if:

\begin{equation}\label{eq:equalized-error}
\forall k_1, k_2 \in [K]: \quad
\Pr \left[ h(x) \neq y \, \vert \, z_{k_1} = 1 \right] \approx \Pr \left[ h(x) \neq y \, \vert \, z_{k_2} = 1 \right]
\end{equation}

We first make the following simple, yet important, observation that will allow us to write fairness constraints, usually defined with respect to binary valued group membership, using a real valued proxy.

\begin{clm}
For every $k \in [K]$, we have
\begin{equation}\label{eq:observation}
    \Pr \left[ h(x) \neq y \, \vert \, z_k =1 \right] = \frac{\E \left[ z_k \1 \left[ h(x) \neq y \right] \right]}{\E \left[  z_k \right]}
\end{equation}
\end{clm}

\ifdraft
\begin{proof}
We have
\begin{align*}
    \Pr \left[ h(x) \neq y \, \vert \, z_k =1 \right] &= \frac{\Pr \left[ z_k = 1, h(x) \neq y \right]}{\Pr \left[ z_k =1 \right]} \\
    & = \frac{\E \left[ \1 \left[ z_k = 1 \right] \1 \left[ h(x) \neq y \right]\right] }{\E \left[ \1 \left[ z_k = 1 \right] \right]} \\
    &= \frac{\E \left[ z_k \1 \left[ h(x) \neq y \right] \right]}{\E \left[  z_k \right]}
\end{align*}
\end{proof}
\fi

Observe that the expression on the right hand side of Equation~\eqref{eq:observation} could be evaluated even if the sensitive feature labels $z$ were real valued rather than binary. We exploit this to evaluate these equalized error fairness constraints with our real valued proxies $\hat z$. Observe that if we have a proxy $\hat{z} \in \Gs$, such that for a particular classifier $h \in \Hs$:
\begin{equation}\label{eq:condition0}
\forall k \in [K]: \quad
\frac{\E \left[ z_k \1 \left[ h(x) \neq y \right] \right]}{\E \left[  z_k \right]} \approx \frac{\E \left[ \hat{z}_k (x) \1 \left[ h(x) \neq y \right] \right]}{\E \left[  \hat{z}_k (x) \right]}
\end{equation}
then if $h$ satisfies proxy fairness constraints defined by the proxy $\hat{z}$, i.e., constraints of the form:
\begin{equation}\label{eq:proxy_constraints0}
\forall k_1, k_2 \in [K]: \quad
\frac{\E \left[ \hat{z}_{k_1} (x) \1 \left[ h(x) \neq y \right] \right]}{\E \left[  \hat{z}_{k_1} (x) \right]} \approx \frac{\E \left[ \hat{z}_{k_2} (x) \1 \left[ h(x) \neq y \right] \right]}{\E \left[  \hat{z}_{k_2} (x) \right]}
\end{equation}
it will also satisfy the original fairness constraints with respect to the real sensitive groups $z$ and vice versa (Equation~\eqref{eq:equalized-error}). If the condition in Equation~\eqref{eq:condition0} is satisfied for \textit{every} $h \in \Hs$, then the proxy fairness constraints (Equation~\eqref{eq:proxy_constraints0}) can without loss be used to \textit{optimize} over all fair classifiers in $\Hs$. With this idea in mind, we can formally define a (good) proxy. The constraints we ask for can be interpreted as so-called \textit{multiaccuracy} or \textit{mean consistency} constraints as studied by \cite{multiaccuracy,momentmulti}, defined over the \textit{error regions} of hypotheses in the class $\Hs$: $\{\{(x,y) : h(x) \neq y\} : h \in \Hs\}$.

We will consider two different settings for modelling a multiplicity of downstream learning problems: 1) when there exists a distribution over $\F$ and we want our guarantee to hold with high probability over a draw of $f$ from this distribution, and  2) when we want our guarantee to hold for every $f \in \F$.

\begin{definition}[Proxy]\label{def:proxy}
Fix a distribution $\Ps$ over  $(\X \times \Z)$  and a distribution $\Qs$ over $\F$. We say $\hat{z}$ is an $(\alpha, \beta)$-proxy for $z$ with respect to $(\Ps, \Qs)$, if with probability $1-\beta$ over the draw of $f \sim \Qs$: for all classifiers $h \in \Hs$, and all groups $k \in [K]$,
\[
\left\vert \frac{\E_{(x,z) \sim \Ps} \left[ z_k \1 \left[ h(x) \neq f(x,z) \right] \right]}{\E_{(x,z) \sim \Ps} \left[  z_k \right]} - \frac{\E_{(x,z) \sim \Ps} \left[ \hat{z}_k (x) \1 \left[ h(x) \neq f(x,z) \right] \right]}{\E_{(x,z) \sim \Ps} \left[  \hat{z}_k (x) \right]} \right\vert \le \alpha
\]
If the above condition holds for every $f \in \F$, we say $\hat{z}$ is an $\alpha$-proxy with respect to $\Ps$. When providing in sample guarantees, we take the distributions to be the uniform distributions over the  data set. When distributions are clear from context, we simply write that $\hat z$ is an $(\alpha, \beta)$-proxy.
\end{definition}

Do such proxies exist? We first show the existence of perfect proxies, under the assumption that the sensitive features and the labels are conditionally independent given the other features. Note that this conditional independence assumption can be satisfied in a number of ways --- and in particular is always satisfied if \textit{either} the sensitive features or the labels can be determined as a function of the non-sensitive features --- even if the relationship is arbitrarily complex. For example this will be the case for prediction tasks in which human beings are near perfect. The proxy that we exhibit below is the conditional expectation defined over the underlying joint distribution on $x$ and $z$ and hence will generally not be learnable from polynomially sized samples. Subsequently, we will demonstrate that we can obtain proxies learnable with modest sample complexity. We note that perfect proxies always exist (without requiring a conditional independence assumption) for statistical parity fairness -- see the appendix.

\begin{clm}[Existence of a Proxy]
\label{clm:existence}
For any distribution $\Ps$ over $\X \times \Z$, $\hat{z}(x) = \E \left[z \,| \, x \right]$ is an $\alpha$-proxy with respect to $\Ps$, for $\alpha = 0$, provided that $z$ and $y$ are independent conditioned on $x$.
\end{clm}

\ifdraft
\begin{proof}
Fix $f \in \F$, $h \in \Hs$, and $k \in [K]$. We have that
\[
\E_{(x,z) \sim \Ps} \left[  \hat{z}_k (x) \right] = \E_{x \sim \Ps_\X} \left[  \hat{z}_k (x) \right] = \E_{x \sim \Ps_\X} \left[  \E \left[z_k \, | \, x \right] \right] = \E_{(x,z)} [z_k ]
\]
Also, note that $y= f(x,z)$, and that
\begin{align*}
    \E_{(x,z) \sim \Ps} \left[ \hat{z}_k (x) \1 \left[ h(x) \neq f(x,z) \right] \right] &= \E_{(x,z)} \left[ \E \left[z_k \, | \, x \right] \1 \left[ h(x) \neq y \right] \right] \\
    &= \E_{(x,z)} \left[ \E \left[z_k \1 \left[ h(x) \neq y \right] \, | \, x \right] \right] \\
    &= \E_{(x,z)} \left[z_k \1 \left[ h(x) \neq y \right] \right] \\
    &= \E_{(x,z)} \left[z_k \1 \left[ h(x) \neq f(x,z) \right] \right]
\end{align*}
completing the proof. The second equality holds because of the assumption that conditional on $x$, $y$ and $z$ are independent.
\end{proof}
\fi

\paragraph{Modelling the Proxy Learner (PL)}
The PL wants to learn a proxy in $\hat{z} \in \Gs^K$ as defined in Definition~\ref{def:proxy}. 

Solving this problem requires the knowledge of distributions; however, typically we will only have samples. Therefore, we assume the PL has access to a data set, which consists of two components: 1) $S = \{ (x_i, z_i) \}_{i=1}^n$ which is a sample of $n$ individuals from $\X \times \Z$ represented by their non-sensitive features and sensitive attributes. Throughout we will take $S$ to be $n$ $i.i.d.$ draws from the underlying distribution $\Ps$. 2) $F = \{ f_j \}_{j=1}^m$ which is a sample of $m$ labeling functions (or \textit{learning tasks}) taken from $\F$. The PL does not observe the actual functions $f_j \in \F$ but instead observes the realized labels of functions in $F$ on our data set of individuals $S$: $Y = \{ y_{ij} = f_j (x_i, z_i) \}_{i,j}$. The \textit{empirical} problem of the PL is to find a proxy $\hat{z}$ with respect to the observed data sets.

In this paper we have the PL optimize  squared error subject to the constraints given by the definition of a proxy:
\begin{mini}|l|
{\hat{z}_k \in \Gs}{\frac{1}{n}\sum_{i=1}^{n} \left( z_{ik} - \hat{z}_k (x_i) \right)^2}{}{}
\addConstraint{\frac{\sum_{i=1}^n z_{ik} \1 \left[  h(x_i) \neq y_{ij} \right]}{\sum_{i=1}^n z_{ik}  } = \frac{\sum_{i=1}^n \hat{z}_{k} (x_i) \1 \left[  h(x_i) \neq y_{ij} \right]}{\sum_{i=1}^n \hat{z}_{k} (x_i)}}{}{, \ \forall j \in [m], h \in \Hs}
\label{eqn:program1}
\end{mini}
Note this formulation gives us a decomposition of learning $\hat{z} = (\hat{z}_1, \ldots, \hat{z}_K) \in \Gs^K$ into learning each component $\hat{z}_k \in \Gs$ separately. The squared error objective is not strictly necessary (the constraints encode our notion of a good proxy on their own), but encourages the optimization towards the conditional label distribution of $z$ given $x$, which we showed in Claim \ref{clm:existence} is a good proxy. In our experiments we find this to be helpful.

\paragraph{Modelling the Downstream Learner (DL)} The DLs want to solve fair learning problems using models in some class $\Hs \subseteq \{h: \X \to \Y\}$ subject to the equalized error fairness constraint given in Equation~\eqref{eq:equalized-error}. The DL does not have access to the sensitive attribute $z$ and instead is given the proxy $\hat z \in \Gs^K$  learned by the PL. Thus, for a given learning task represented by some $f \in \F$ (determining the label $y = f(x,z)$), the DL solves the following  learning task subject to proxy fairness constraints.
\begin{mini}|l|
{h \in \Hs}{\E \left[ \text{err} \left( h ; (x,y)\right)\right] }{}{}
\addConstraint{\frac{\E \left[ \hat{z}_{k_1} (x) \1 \left[ h(x) \neq y \right] \right]}{\E \left[  \hat{z}_{k_1} (x) \right]} \approx \frac{\E \left[ \hat{z}_{k_2} (x) \1 \left[ h(x) \neq y \right] \right]}{\E \left[  \hat{z}_{k_2} (x) \right]}}{}{, \ \forall k_1, k_2 \in [K]}
\label{eqn:program3}
\end{mini}
where $\text{err}$ is some arbitrary objective function, and all expectations here are taken with respect to a draw of an individual $(x,z)$ from $\Ps$. Observe that if $\hat z$ is an $\alpha$-proxy, then this is equivalent to solving the original fairness constrained learning problem (defined with respect to the true demographic features $z$) in which the fairness constraints have slack at most $2\alpha$. We remind the reader that our focus in this paper is to solve the problem of the PL, and hence, we avoid standard issues that the DL will face, such as relating empirical and distributional quantities (these issues are identical whether the DL uses the sensitive features $z$ directly or a proxy $\hat z$). 

\paragraph{Game Theory and Online Learning Basics.}
In our analysis, we rely on several key concepts in game theory and online learning which we summarize here. Consider a zero-sum game between two players, a Learner with strategies in $S_1$ and an Auditor with strategies in $S_2$. The payoff function of the game is $U: S_1 \times S_2 \rightarrow \R_{\ge 0}$.

\begin{definition}[Approximate Equilibrium]\label{def:nuapprox}
A pair of strategies $(s_1, s_2) \in S_1 \times S_2$ is said to be a $\nu$-approximate minimax equilibrium of the game if the following conditions hold:
\[
 U(s_1, s_2) - \min_{s'_1 \in S_1}  U(s'_1, s_2)  \le \nu,
\quad
\max_{s'_2 \in S_2}  U(s_1, s'_2) -  U(s_1, s_2)  \le \nu
\]
\end{definition}

Freund and Schapire \cite{Freund} show that if a sequence of actions for the two players jointly has low \textit{regret}, then the uniform distribution over each player's actions forms an approximate equilibrium:

\begin{thm}[No-Regret Dynamics \cite{Freund}]\label{thm:noregret}
    Let $S_1$ and $S_2$ be convex, and suppose  $U(\cdot, s_2): S_1 \to \R_{\ge 0}$ is convex for all $s_2 \in S_2$ and $U(s_1, \cdot): S_2 \to \R_{\ge 0}$ is concave for all $s_1 \in S_1$. Let $(s_1^1, s_1^2, \ldots, s_1^T)$ and $(s_2^1, s_2^2, \ldots, s_2^T)$ be  sequences of actions for each player. If for $\nu_1,\nu_2 \ge 0$, the regret of the players jointly satisfies
    \[
    \sum_{t=1}^T U(s_1^t, s_2^t) - \min_{s_1 \in S_1} \sum_{t=1}^T U(s_1, s_2^t) \le \nu_1 T,
    \quad
    \max_{s_2 \in S_2} \sum_{t=1}^T U(s_1^t, s_2) - \sum_{t=1}^T U(s_1^t, s_2^t) \le \nu_2 T
    \]
then  the pair $(\bar{s}_1, \bar{s}_2)$ is a $(\nu_1+\nu_2)$-approximate equilibrium, where      $\bar{s}_1 = \frac{1}{T}\sum_{t=1}^T s_1^t \in S_1$ and $\bar{s}_2 = \frac{1}{T}\sum_{t=1}^T s_2^t \in S_2$ are the uniform distributions over the action sequences.
\end{thm}

\begin{comment}
\subsection{Organization}
\saeed{re-write this}The rest of the paper is organized as follows. First we consider the case in which we have samples of learning problems from $\F$ and wish to learn $(\alpha,\beta)$-proxies for $\F$. In Section \ref{sec:lin}, we give an algorithm for learning a \textit{linear} proxy $\hat z$ (when one exists). We handle the general case (in which $\hat z$ can be arbitrary, so long as we have a regression oracle for it) in Section \ref{sec:general}. In Section \ref{sec:kahuna} we show how to learn an $\alpha$-proxy for the entire class $\F$ given an appropriate classification oracle. These results are all for empirical (in-sample) optimization. In Section \ref{sec:generalization}, we prove generalization theorems for proxies which allow us to lift our learning guarantees to out-of-sample statements. 
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> New Folder With Items/generalization_facct.tex <==
In this section, we provide generalization guarantees for a proxy using a \textit{uniform convergence} approach.

First, in Theorem~\ref{thm:gen-x}, we consider the case where there is no distribution over the class of labeling functions $\F$, and we want to form a good proxy for \textit{every} labelling function in $\F$; in particular, we show how many samples in $S \sim \Ps^n$ are required to guarantee (with high probability over $S$) that \textit{every} $\hat z$ that is a good proxy with respect to the sample $S$ is also a good proxy with respect to the underlying distribution of the data points $\Ps$. Second, in Theorem~\ref{thm:gen-xf}, we consider the case where there is a distribution $\Qs$ over the class of labeling functions $\F$, in addition to the distribution $\Ps$ over individuals; in particular, we show how many samples in $S \sim \Ps^n$ and $F \sim \Qs^m$ are required to guarantee (with high probability over $S$ and $F$) that \textit{every} $\hat z$ that is a good proxy with respect to the sample $(S,F)$ is also a good proxy with respect to the distributions $(\Ps, \Qs)$. We point out that our uniform convergence bounds are taken over the entire $\Delta (\Gs)^K$, not only $\Gs^K$, because our algorithm outputs an object in $\Delta (\Gs)^K$.

It turns out that the sample complexity of learning such proxies can be characterized by the \textit{pseudo-dimension} ($Pdim$) of the proxy class $\Gs$, which is a standard notion used in the learning theory literature (see for e.g. \cite{haussler}) to measure the complexity of a \textit{real-valued} function class. While we provide the formal definition of pseudo-dimension in the appendix, we note a couple of facts regarding this notion. First, pseudo-dimension generalizes the notion of \textit{VC dimension} ($VCdim$) which is typically used to measure the complexity of \textit{binary} function classes.

\begin{fact}[\cite{haussler}]\label{fact:pseudo-vc}
If $\Hs \subseteq \{ h: \X \to \{0,1\} \}$, then $Pdim (\Hs) = VCdim (\Hs)$.
\end{fact}

Second, if $\Gs$ is a class of $d$-dimensional \textit{linear} proxies, then $Pdim(\Gs) = d$ 

\begin{fact}[\cite{haussler}]\label{lem:vectorspace}
If $\Gs \subseteq \{ g: \X \to \R \}$ forms a vector space of dimension $d$, then $Pdim (\Gs) = d$.
\end{fact}

 With this notion of pseudo-dimension in hand, we formally state our first generalization theorem below in Theorem~\ref{thm:gen-x}. We note that in addition to the pseudo-dimension of $\Gs$, our sample complexity bound depends on the VC dimension of $\Hs$ and $\F$ as well because we take a uniform convergence approach that requires bounding the difference of empirical and distributional expectations appearing in the definition of the proxy, for \textit{all} classifiers $h \in \Hs$, and \textit{all} learning tasks $f \in \F$. The sample complexity bound will further depend polynomially on $M$ (a uniform upper bound for functions in $\Gs$), $\mu$ (smallest probability measure of groups), and $\mu_\Gs$ (smallest probability measure of groups, determined by proxies in $\Gs$). The proof of this theorem is in the appendix.

\begin{thm}[Generalization over $\Ps$]\label{thm:gen-x}
Fix any $\epsilon$ and $\delta$. Fix a distribution $\Ps$ over $\X \times \Z$. Suppose $Pdim (\Gs) = d_\Gs$, $VCdim(\F) = d_\F$, and $VCdim(\Hs) = d_\Hs$. We have that with probability at least $1-\delta$ over $S \sim \Ps^n$, every $\hat z$ that is an $\alpha$-proxy with respect to the data set $S$ is also an $(\alpha + \epsilon)$-proxy with respect to the underlying distribution $\Ps$, provided that
\[
n = \tilde{\Omega} \left( \frac{M^2 \left( d_\Gs + \max \left\{ d_\Hs, d_\F \right\}  + \log \left( K / \delta \right) \right)}{\mu \mu_\Gs^2 \left( \min \left\{ \mu, \mu_\Gs \right\} \right)^2 \epsilon^2} \right)
\]
where
$
\mu = \min_{1 \le k \le K} \E_{(x,z) \sim \Ps} \left[ z_k \right], \ \mu_\Gs = \inf_{\hat z \in \Gs} \left\{  \min_{1 \le k \le K} \E_{(x,z) \sim \Ps} \left[ \hat{z}_k (x) \right] \right\}
$.
\end{thm}

\begin{rmk}
We remark that Theorem~\ref{thm:gen-x} subsumes the case when there is only one, or more generally, finitely many learning tasks, because it is known that if $| \F | < \infty$, then we have $d_\F \le \log \left( | \F | \right)$.
\end{rmk}


We note that the sample complexity bound of Theorem~\ref{thm:gen-x} grows with the VC dimension of $\F$, i.e., we are assuming $\F$ has bounded complexity ($d_\F < \infty$). In our next generalization theorem, we consider the setting where there is a distribution over $\F$ from which an $i.i.d.$ sample is collected. This distributional modeling allows us to make no assumption on the complexity of $\F$, i.e., $\F$ can have $d_\F = \infty$. This allows us to handle real labels, without the need to make any assumptions about their underlying complexity. The proof of Theorem~\ref{thm:gen-xf} is provided in the appendix.

\begin{thm}[Generalization over $\Ps$ and $\Qs$]\label{thm:gen-xf}
Fix any $\epsilon$, $\delta$, and $\beta$. Fix a distribution $\Ps$ over $\X \times \Z$, and a distribution $\Qs$ over $\F$. Suppose $Pdim (\Gs) = d_\Gs$, and $VCdim(\Hs) = d_\Hs$. We have that with probability at least $1-\delta$ over $S \sim \Ps^n$ and $F \sim \Qs^m$, every $\hat z$ that is an $(\alpha, 0)$-proxy with respect to the data set $(S, F)$ is also a $((\alpha + \epsilon) / \beta, \beta )$-proxy with respect to the underlying distributions $(\Ps, \Qs)$, provided that
\[
n = \tilde{\Omega} \left( \frac{ M^{2} \left( d_\Gs + \max \left\{ d_\Hs, \log \left( m \right) \right\}  + \log \left( K / \delta \right) \right)}{ \mu \mu_\Gs^2 \left( \min \left\{ \mu, \mu_\Gs \right\} \right)^2 \epsilon^2} \right),
 \ m = \tilde{\Omega} \left( \frac{ M^{2} \left( K d_\Gs \log \left( \left\vert \text{supp} (\Ps) \right\vert \right) + \log \left( 1 / \delta \right) \right) }{ \mu_\Gs^2 \left( \min \left\{ \mu, \mu_\Gs \right\} \right)^2 \epsilon^4} \right)
\]
where $\text{supp} (\Ps)$ is the support of $\Ps$, and $\mu$ and $\mu_\Gs$ are defined as in Theorem~\ref{thm:gen-x}.
\end{thm}

\begin{rmk}
Our bounds contain the term $\mu_{\Gs}$ because they are algorithm independent uniform convergence bounds. The algorithms we give in this paper however always produce a $\hat{z}$ that satisfies $\E_{S} \left[ \hat{z}_k (x) \right] \ge (1/2)\E_{S} \left[ z_k \right]$ in sample. Together with standard arguments, this allows us to give generalization guarantees for our algorithms that remove the dependence on $\mu_\Gs$. Technically, this follows from applying our uniform convergence theorems to the class $\Gs^K(\mu) \equiv \{ \hat{z} \in \Gs^K: \forall k, \, \E_{(x,z) \sim \Ps} \left[ \hat{z}_k (x) \right] = \Omega (\mu) \}$.
\end{rmk}
